Exciton dynamics in equilibrium and nonequilibrium regimes

The bound electron-hole pairs known as excitons govern the optical properties of insulating solids. While their behavior in equilibrium is well-understood theoretically, the nonequilibrium regime at high excitation densities-where phenomena like electron-hole liquids emerge - is less explored. This thesis presents a first-principles study of excitons in two-dimensional materials. We use the GW approximation and the Bethe-Salpeter equation to investigate their properties from equilibrium to nonequilibrium conditions. We first demonstrate how increasing photo-excited carrier density leads to a redshift-blueshift crossover of excitons. We then show that electron-phonon interactions critically modify optical spectra and exciton lifetimes at finite temperatures. Finally, we unify these effects to demonstrate the formation of an electron-hole liquid phase above a critical carrier density and below a critical temperature. Our work identifies how enhanced Coulomb interactions in two dimensions can stabilize this phase at significantly higher temperatures, proposing promising material candidates for observing these collective states.

==> Certificate.tex <==

\thispagestyle{fancy}
\makeatletter%
\long\def\@makefnmark{%
	\hbox {{\normalfont \@thefnmark }}}%
\makeatother


\makeatletter%
\long\def\@makefntext#1{%
	\parindent 1.5em\noindent \hb@xt@ 1.5em{\hss [\@makefnmark] }#1}%
\makeatother

\begin{flushleft}
\includegraphics[scale=.4]{logoiitk.pdf}
\end{flushleft}
\centerline{\Large\bf CERTIFICATE}
\hrulefill
\bigskip

\begin{quote}
It is certified that the work contained in the thesis titled \textbf{\textit{``Exciton dynamics in equilibrium and nonequilibrium regimes''}}, by \textbf{\textit{Pushpendra Kumar Yadav},} has been carried out under my supervision and that this work has not been submitted elsewhere 
for a degree.

\vspace{30mm}
\begin{flushright} % Use the flushright environment for right alignment
	\begin{tabular}[c]{ll}
		\vspace{2.1mm}
		{} & {\bf  Prof. Amit Agarwal}\\
		\vspace{2.1mm}
		{} & {\bf  Department of Physics} \\
		{} & {\bf Indian Institute of Technology Kanpur}
	\end{tabular}

	\vspace{10mm} % Adjust the space between the table and the date if needed
	
	February, 2024
\end{flushright}


\end{quote}
\hrulefill




==> OnlySynopsis/synopsis_py.tex <==
% !TEX root = thesis_revised.tex

\thispagestyle{fancy}
\makeatletter%
\long\def\@makefnmark{%
\hbox {{\normalfont \@thefnmark }}}%
\makeatother


\makeatletter%
\long\def\@makefntext#1{%
  \parindent 1.5em\noindent \hb@xt@ 1.5em{\hss [\@makefnmark] }#1}%
\makeatother

\centerline{\Huge\bf Synopsis}
\vskip 1.0cm 
\begin{quote}
	\begin{tabular}[]{p{5.5cm}cp{9.0cm}}
		Name				&:	&{\bf Pushpendra Kumar Yadav}\\[0.5em]
		Roll No.			&:	&{\bf 18209268 }\\[0.5em]
		Degree for which submitted	&:	&{\bf Doctor of Philosophy}\\[0.5em]
		Department			&:	&{\bf Physics}\\[0.5em]
		Title of the Thesis 		&:	&{\bf Exciton dynamics in equilibrium}\\
		& &{\bf and nonequilibrium regimes}\\
		
		\\
		
		Thesis Supervisor		&:	&{\bf Prof. Amit Agarwal} \\ 
		\\[0.5em]
		
		%		\\
		Month and year \\ of submission	&:	&{\bf January, 2024}\\[0.0em]
	\end{tabular}
\end{quote}
\hrule
%\hrulefill
\vskip 1.0 cm

Interaction among the photo-excited electrons and holes in an insulating solid leads to the formation of a bound state of an electron-hole pair called exciton~[\footnote{{L. J. Sham and T. M. Rice}, {\em Phys. Rev.}, {\bf 144}, 708~(1966)}, \footnote{{G. Strinati}, {\em Phys. Rev. B}, {\bf 29}, 5718~(1984)}]. The excitons govern most of the optical responses and explain several fundamental phenomena in condensed matter. By incorporating the electron-hole correlations at absolute zero temperature and low electron-hole pair density in the excited state, \textit{ab-initio} based theoretical study of optical excitations predict reasonably accurate optical absorption and emission [\footnote{{M. S. Hybertsen and S. G. Louie}, {\em Phys. Rev. Lett.}, {\bf 55}, 1418~(1985)}]. However, some recent experiments have probed the impact of exciton-exciton interactions by increasing the pump fluence or photo-excited carrier density, bringing the electron-hole system into a nonequilibrium regime [\footnote{{Sie, E. J. {\em et. al.}}, {\em Nano Lett.}, {\bf 17}, 7, 4210–4216~(2017)}]. At finite temperatures, within the nonequilibrium regime, the electron-hole system has been reported to exhibit electron-hole plasma and electron-hole liquid phase in the density-temperature parameter space~[\footnote{{Arp T. B., {\em et. al.}}, {\em Nat. Photon.}, {\bf 13}, 245~(2019)}]. However, the theoretical understanding of these exciting experiments in the nonequilibrium regime is yet to be explored.

In this thesis, we demonstrate the presence of bound excitons in atomically thin two-dimensional materials from first-principle based approach. We estimate the single-particle energies using the GW approximation (GWA) and incorporate the electron-hole correlations via the Bethe-Salpeter equation (BSE). The fundamentals of excitons have been studied in the low excitation density, i.e., in the equilibrium limit. With increasing photo-excited carrier density, we show that the lowest energy exciton in monolayer MoSi$_2$Z$_4$ (Z = N, P, As) follows the redshift-blueshift crossover due to the renormalized exciton binding energies in the nonequilibrium regime. Further, we study temperature-dependent optical absorption and photoluminescence (PL) phenomenon in monolayer aluminum nitride (AlN) in the equilibrium regime. We find that electron-phonon interactions significantly modify the electronic energy, excitonic absorption, emission spectrum, and exciton lifetime. At low temperatures, the PL emission signals exhibit full excitonic thermalization with phonon replica below the indirect exciton energy. Finally, we combined the impact of temperature and electron-hole density and investigated a photo-excited electron-hole system in the nonequilibrium regime. We show that photo-excited electrons and holes in insulators above a critical density and below a critical temperature can condense to form an electron–hole liquid (EHL) phase. However, observing the EHL phase at room temperature is extremely challenging. Here, we propose the monolayer MoSi$_2$Z$_4$ (Z = N, As, P) series of compounds as promising platforms for observing the EHL phase at room temperature. Stronger effective Coulomb interactions in two dimensions help these monolayers stabilize the EHL phase with increased EHL binding energy, transition temperature, and strongly bound excitons. 
%Our findings motivate further exploration of two-dimensional semiconductors for realizing the EHL phase at high temperatures and harness collective phenomena for optoelectronic applications.

In Chapter 1, we introduce the fundamentals of the exciton quasiparticles generated upon optical excitation in insulating materials and their impact on different physical observables in condensed matter. A brief discussion about the types of excitons, the effect of dimensionality, and screening on exciton binding energies follows this. Next, we classify excitons based on optical selection rules as bright and dark excitons and based on their interaction with other charged particles or excitons, such as trion and biexciton complexes and electron-hole droplets. In the latter part of the chapter, we discuss the importance of exciton physics in two-dimensional materials and their usefulness in next generation optoelectronic devices. Briefly, we also discuss the theoretical methods adopted for studying optical excitations in this thesis.

In Chapter 2, we discuss the different formalisms used to explore the electronic structures and optical excitations using first-principles methods. We review the many-body Hamiltonian and its solution within the density functional theory (DFT). Further, to incorporate the electron-self energy, we have adopted the GW (where $G$ stands for the single-particle Green's function and $W$ represents the screened Coulomb potential) approximation to estimate the quasiparticle energies of photo-excited electrons and holes. This is followed by a discussion on the interaction between optically excited electrons and holes leading to the exciton formation and a calculation of the exciton energies and coupled electron-hole wavefunction utilizing the Bethe-Salpeter equation (BSE). Furthermore, to understand the effect of lattice vibrations on optical excitations, we follow the electron-phonon interaction calculation within the density functional perturbation theory and obtain electron-phonon matrix elements. The electron-phonon interaction effects are finally applied to the quasiparticles (electron, hole, and excitons) energy correction, and the role of phonon momentum is utilized to understand the indirect photon emission in the indirect bandgap materials. 


In Chapter 3, we investigate the exciton quasiparticle generated in synthetic monolayers of MoSi$_2$N$_4$, MoSi$_2$As$_4$, and MoSi$_2$P$_4$, upon optical excitation. Going beyond the equilibrium properties, we study the fluence-dependent optical spectra and the emergence of exciton–exiton interaction in the nonequilibrium regime for MoSi$_2$N$_4$.
We unveil the renormalization of the exciton binding energy (BE) of the $A$ and $B$ exciton peaks with increasing photo-generated carrier density in the MoSi$_2$N$_4$ monolayer. The exciton BE shows a redshift with increasing pump fluence or photo-excited charge carrier density. This decrease in the BE arises from screening the excitonic Coulomb potential by the
photo-excited charge carriers. However, the exciton binding energies show a blueshift crossover on further increase in the pump fluence or exciton density. This establishes that excitons in the MoSi$_2$N$_4$ series display an atom-like attractive and repulsive interaction depending on the inter-exciton separation. Furthermore, for the direct band gap MoSi$_2$As$_4$ and
MoSi$_2$P$_4$ monolayers, we accurately predict the fundamental quasiparticle (QP) and optical band gaps with their detailed excitonic character.

In Chapter 4, we predict the impact of electron-phonon coupling on optical absorption, PL emission, and indirect emission mechanism. We utilize first-principle calculations and calculate temperature-dependent optical properties of a planar AlN monolayer. Our investigation demonstrated the effect of electron-phonon (el-ph) interactions, leading to significant renormalization of quasiparticle energies. Specifically, the calculated optical absorption spectra showcases a redshift and decreased dipole oscillator strengths due to the interplay between electronic and vibrational states. Furthermore, we observe phonon-assisted indirect PL emission within the excitonic framework in the ultraviolet regime. The PL emission sustains at higher temperatures ( $\ge$ 300 K). Furthermore, the highlighted role of exciton-phonon interactions extends beyond AlN, emphasizing their importance in group-III nitrides and other two-dimensional materials. 


In chapter 5, we establish potential observation of the EHL phase at room temperature within the monolayer {\formulaN} family. Because of the dimensional confinement and reduced dielectric constant, the monolayer {\formulaN} family host strongly bound excitons with exciton binding energy of the order of 1 eV, as discussed in Chapter 3. Since the critical temperature of the EHL phase depends directly on the exciton binding energy ($T_c \sim 0.1E_b$), and therefore {\formulaN} family host EHL phase above a critical exciton density ($n_c$). This prediction marks a significant departure from conventional limitations associated with cryogenic conditions, introducing the observation of the EHL phase in these materials at room temperature. The higher impact of the Coulomb interactions in two dimensions helps these monolayers support the EHL phase with an increased EHL binding energy and transition temperature, along with strongly bound excitons. Our findings motivate further exploration of the {\formula} monolayers for realizing the EHL phase at high temperatures to harness collective
phenomena for optoelectronic applications. %In another experimental collaborative study, we predict the EHL phase in bulk CsPbBrI$_2$ nanocrystals at room temperature. The stability of the EHL phase in the bulk CsPbBrI$_2$ is supported by the strong electron-phonon interaction, leading to strong electron-hole correlation effects. Furthermore, our study will hopefully broaden the understanding of carrier dynamics in ﬂourishing metal-halide perovskite material and {\formula} monolayers, which will help to enhance the light-matter interaction in photovoltaics, optoelectronic devices.


Finally, we summarize the main findings of our work in Chapter 6, followed by a discussion of future prospects.


==> acknowledge_backup.tex <==
% !TEX root = thesis_revised.tex

\thispagestyle{plain}
\begin{center}
	{\Huge \bf Acknowledgements}
\end{center}

\vskip 50pt
"Life is a journey" feels more realistic now. When I came to this beautiful campus of IIT Kanpur in January 2019 for my Ph.D., it felt like a home here. Just a couple of my undergraduate friends were like a trigger for a chain reaction of making friends for life in the campus. Their company and cheerfulness made me fall in love for this vibrant and soulful campus and spent five most beautiful years of my life. It has been an honor to pursue physics within this intellectually rich research environment of IITK, which has helped me grow academically and learn life lessons. Now, as this beautiful journey is about to end, I would like to express my heartfelt gratitude to everyone who has been a part of it.

First and foremost, I sincerely thank my thesis supervisor, Prof. Amit Agarwal. Without him, I could not accomplish what I have so far. I joined Prof. Amit for my PhD in January 2019. Throughout these years, I have learned a lot of lessons, academic and non-academic, which I will remember for my life. Discussing physics with him has always been a learning experience for me. His guidance in breaking complex problems and calculations in the easiest possible way and his positive perspective has helped me transform into a different personality. His open-mindedness for new projects and learning new tools has always encouraged me to learn new things that immensely helped my Ph.D. training. He has played a crucial role in improving my academic writing and project management skills with his constant advice. He is a great mentor, a thoughtful advisor, and an excellent motivational speaker. He always reminded me of my privileges as a researcher whenever I faced ups and downs during these years. I would also like to thank Prof. Amit and his family for the cheerful moments shared during Diwali and several other dinner occasions.

I want to express my sincere gratitude to Prof. K V Adarsh and Prof. Subham Majumdar. Working with these outstanding experimental physicists during our collaborative efforts provided me with valuable insights into the experimental aspects of condensed matter physics. I extend my heartfelt thanks to Prof. Sitangshu Bhattacharya and Prof. Bramhachari Khamari for their guidance in learning about the theoretical understanding of exciton physics. Their persistent support in learning computational methods has been a pillar of strength for me.

I am grateful to the Late Prof. Amit Dutta, Prof. Manoj K. Harbola, Prof. Arijit Kundu, Prof. Adhip Agarwala, Prof. Sudeep Ghosh, and Prof. Koushik Pal for providing invaluable feedback on my work during seminars and peer reviews. Their insights have significantly contributed to the refinement of my research.

I extend my sincere gratitude to Dr. Gyan Prakash, Dr. Sougata Mardanya, Dr. Barun Ghosh, Dr. Atasi Chakraborty for their constant support, encouragement, and insightful technical and conceptual discussions. They have served as mentors, guiding me through the challenges in academics and life. I also want to express my appreciation to other collaborators, namely Suman Mondal, Ajay Poonia, Dr. Imran Ahamed, Riyanka Karmakar, and Pravrati Taank, from whom I have gained valuable insights into various aspects of condensed matter physics.

I am grateful to my friends and colleagues in the QTT group Kamal, Raihan da, Debottam, Debasis, Maneesh, Nirmalya, Sunit, Harsh, Sanjay, Dibyanandan, Koushik, and Sayan. Our daily tea break has always been a delightful time when we step outside to research, share jokes, discuss life, and lighten the mood as an experience I will always cherish. Having Kamal, Debasis, and Debottam as friends in the group has been a blessing for me. Our discussions extended beyond physics, involving random dinner outings and supporting each other whenever needed. I am grateful to everyone in the group for their help in my PhD seminar and thesis.

I am thankful to my friends at IITK, Rohit, Tahir, Kishori, Ashish, Poonam, Hari, Vinayak, Pooja, Soumyadeep, Ayesha, Swati, Santu, Pranesh, Ekta, Suraina, Suman, Ankur for creating the most memorable moments during midnight birthday celebrations, especially in the chilling months of December and January. I am also grateful to my friends from the 103D Lab Samrat, Vikash, Bheem, Arunava, Joy, Abhijit and others for for the philosophical and humorous discussions both in and outside the lab. I extend my sincere thanks to my friends at Hall-XI, Kamal, Yogesh, Rohit, Himanshu, Bashab for late night parties and for the best adventuras memory of playing vollyball games in the coldest nights of Kanpur. I also very gratful to Ashok bhaiya, Gaganjot bhaiya,  Shuryakant bhaiya, Samiullah, Saswat, Amitabh, Sanatan, Pankaj, Monu, and Saikat and others for the dinner table discussions which has always helped me feeling livelyhood in Hall XI. I am also very grateful to my college friends Saurabh, Sunil, Dheeraj, Nauratan, Anjanay, Krishna, Uma, Shambhavi, Dipika, Prem, Satya, Shashank, Vivek, Kushagra, and Anand.  

I would also like to express my gratitude to my M.Sc. thesis supervisor, Prof. Ranjit Nanda. I am sincerely thankful to Prof. Pinaki Majumdar for his support and for providing me with opportunities to work with him during and after my master's program. Your guidance has been influential in leading me to where I am today, working in computational condensed matter physics.

I am grateful to all my teachers, specially Mr. Mohan Lal Yadav, who always has been a guardian, a mentor, and a source of inspiration for me. I am also grateful to my childhood friend Sunil and all my classmates throughout my journey who have motivated me to be a better student and a kind human being.

I express my special thanks to Vijaya, my friend and companion, for her unconditional love and support. She has always been there for me, listening, encouraging, and cheering me up whenever I was worried about anything in life. With her, this journey has been more beautiful and full of joys.

Above all, I express my gratitude to my family members. My father has a special impact on my life for providing me with his invaluable support and encouragement, especially for his efforts in waking us up at 4 AM in the morning and making the best tea ever for us so that we could study. He still makes the best tea that I can find anywhere. Special thanks to my mother for her unwavering love and support, and particularly for helping me learn cooking. I am very grateful for my elder brothers for their support, encouragement, and for believing in me. Last but not least, I'm thankful to my younger brother, who has always been there for any help and support I needed, especially for taking care of our parents. Without them, it could not have been easy for me to accomplish my goals. I dedicate my achievements to them.

\begin{flushleft}
	January, 2024 \hfill {Pushpendra Kumar Yadav}
\end{flushleft}


==> decleration.tex <==

\thispagestyle{fancy}
\makeatletter%
\long\def\@makefnmark{%
	\hbox {{\normalfont \@thefnmark }}}%
\makeatother


\makeatletter%
\long\def\@makefntext#1{%
	\parindent 1.5em\noindent \hb@xt@ 1.5em{\hss [\@makefnmark] }#1}%
\makeatother
\renewcommand{\headrulewidth}{0pt}

	\centerline{\Large\bf DECLARATION}
	\hrulefill
	\bigskip
	
	\begin{quote}
		This is to certify that the thesis titled \textbf{\textit{``Exciton dynamics in equilibrium and nonequilibrium regimes''}} has been authored by me. It presents the research conducted by me under the supervision of \textbf{\textit{Prof. Amit Agarwal}}. To the best of my knowledge, it is an original work, both in terms of research content and narrative, and has not been submitted elsewhere, in part or in full, for a degree. Further, due credit has been attributed to the relevant state-of-the-art and collaborations (if any) with appropriate citations and acknowledgements, in line with established norms and practices.
		
		\vspace{30mm}  
		\begin{flushright}
			%\begin{quote}
			\begin{tabular}[c]{ll}
				\vspace{2.1mm}
				%{} & {\bf (Signature of Supervisor)}\\
				{} & {\bf Pushpendra Kumar Yadav}\\
				%\vspace{2.1mm}
				{} & {\bf Programme: Ph.D.}\\
				{} & {\bf Department of Physics} \\
				{} & {\bf Indian Institute of Technology Kanpur}
			\end{tabular}
		
		\vspace{10mm} % Adjust the space between the table and the date if needed
		
		February, 2024
		\end{flushright}
		
	\end{quote}
	\hrulefill




==> diff.tex <==
% !TEX root = thesis_revised.tex

\chapter{Electronic structure theory}
\label{chap2}
\pagestyle{fancy}
The theoretical tools used in this thesis to model the electronic structure of topological semimetals are  (i) DFT based $ab~initio$ calculations (ii) Wannier function based tight-binding modeling and (iii) group theory based symmetry analysis along with the ${\bf k.p}$ perturbation theory-based model Hamiltonian approach. In the recent past, DFT based $ab~initio$ techniques together with the Wannier function based tight-binding approach has proven to be extremely useful for exploring topological materials.~\cite{martin2004,march1983,sholl2011density,prasad2013,Hasan10,Bansil16} Ideally, DFT based computations are not dependent on any empirical parameters, and therefore one can predict the topological properties of a system starting only from the crystal structure data. This makes DFT a powerful tool for identifying and characterizing new topological materials. In fact, in the recent past,  many of the non-trivial topological materials \DIFdelbegin \DIFdel{are }\DIFdelend \DIFaddbegin \DIFadd{were }\DIFaddend first theoretically predicted using the DFT based calculations, \DIFdelbegin \DIFdel{which later got }\DIFdelend \DIFaddbegin \DIFadd{and they were later }\DIFaddend verified experimentally. 

In this chapter, we briefly review the formulations of DFT and Wannier based tight-binding approach. In Sec.~\ref{Elec_Ham}, we discuss about the simplification of the Hamiltonian of a many-electron system by various approximations. In Sec.~\ref{DFT}, we introduce various concepts of DFT. We start with the Kohn-Sham theorem and extend the discussion to review different approximations involved in the calculation of exchange-correlation energy functionals. Next, we discuss about the plane-wave basis and the pseudopotentials methods. In Sec.~\ref{wann}, we discuss about the Wannier functions. We review various properties of the Wannier functions and explain the methods to obtain surface states using the Wannier function based tight-binding formalism.

\section{A system with many electrons}\label{Elec_Ham}
The Hamiltonian for a system with a number of ions and electrons can be expressed as,
%
\be\label{Ham1}
H=T_I+T_E+V_{II}+V_{EE}+V_{IE}~.
\ee
%
where, and $T_I$ and $T_E$ denote the kinetic energy of the ions and the electrons, respectively, $V_{II}$, $V_{EE}$, and $V_{IE}$ are the ion-ion, electron-electron, and  ion-electron parts of the Coulomb interaction, respectively~\cite{prasad2013,vanderbilt2018berry}. These terms can be written in the explicit forms as,
%
\bearr
T_{I} &=& -\frac{\hbar^2}{2M}\sum_I \mathbf{\nabla}^2_I~~,\\
T_E &=& ~~-\frac{\hbar^2}{2m}\sum_i \mathbf{\nabla}^2_i,\\
V_{EE}&=& \frac{1}{2} \sum_{\substack{i,j \\ i\neq j}} \frac{e^2}{|\mathbf{r}_i-\mathbf{r}_j|}~~,\\
V_{II}&=& \frac{1}{2} \sum_{\substack{I,J \\ I\neq J}} \frac{(Ze)^2}{|\mathbf{R}_I-\mathbf{R}_J|}~~,\\
V_{IE}&=& - \sum_{\substack{i,I}} \frac{Ze^2}{|\mathbf{r}_i-\mathbf{R}_I|}~~.
\eearr
\DIFdelbegin \DIFdel{Where, m and M denotes }\DIFdelend \DIFaddbegin \DIFadd{Here, $m$ and $M$ denote }\DIFaddend the mass of the electrons and ions, respectively, \DIFdelbegin \DIFdel{Z }\DIFdelend \DIFaddbegin \DIFadd{and $Z$ }\DIFaddend is the nuclear charge. \DIFdelbegin \DIFdel{The }\DIFdelend \DIFaddbegin \DIFadd{Additionally, }\DIFaddend $\mathbf{r}$ and $\mathbf{R}$ \DIFdelbegin \DIFdel{represents }\DIFdelend \DIFaddbegin \DIFadd{represent }\DIFaddend the electronic and ionic coordinates, respectively. Combining all the terms, the full Hamiltonian of a many-electron system is given by 
\bearr
H= -\frac{\hbar^2}{2M}\sum_I \mathbf{\nabla}^2_I -\frac{\hbar^2}{2m}\sum_i \mathbf{\nabla}^2_i + \frac{1}{2} \sum_{\substack{i,j \\ i\neq j}}  \frac{e^2}{|\mathbf{r}_i-\mathbf{r}_j|} + \frac{1}{2} \sum_{\substack{I,J \\ I\neq J}} \frac{(Ze)^2}{|\mathbf{R}_I-\mathbf{R}_J|} 
 - \sum_{\substack{i,I}} \frac{Ze^2}{|\mathbf{r}_i-\mathbf{R}_I|}~. \nonumber\\ 
\eearr
Therefore, the time-independent Schrodinger \DIFdelbegin \DIFdel{'s }\DIFdelend equation for this system can be written as,
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend %DIF > 
\be\label{SE1}
H~ \phi =E_{tot}~\phi 
\ee
 %
{Here, $E_{tot}$ and $\phi$ represent the eigenvalues and the many-body \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend of this ion-electron system. For a real system with $\approx 10^{23}$ number of electrons and ions \DIFaddbegin \DIFadd{solving }\DIFaddend this equation is \DIFdelbegin \DIFdel{not possible to solve }\DIFdelend \DIFaddbegin \DIFadd{extremely difficult }\DIFaddend with today's \DIFdelbegin \DIFdel{computers. }\DIFdelend \DIFaddbegin \DIFadd{technology. %DIF > not possible to solve with today's computers.
}\DIFaddend 

The first approximation to solve Eq.~\ref{SE1}, \DIFdelbegin \DIFdel{comes through }\DIFdelend \DIFaddbegin \DIFadd{decouples the electronic and the ionic degrees of freedoms and is called }\DIFaddend the Born-Oppenheimer approximation \cite{born1927}. According to this approximation, since the ions in a typical solid move much slowly compared to the electrons, one can decouple the motion of electrons and ions. In other words, the total \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend can be written as a product of electronic and ionic \DIFdelbegin \DIFdel{wavefunctions}\DIFdelend \DIFaddbegin \DIFadd{wave-functions}\DIFaddend , i.e.,
 %
 \be\label{Psi_BO}
 \phi = \psi(\mathbf{r},\mathbf{R}) \chi_{I}(\mathbf{R}).
 \ee 
\DIFdelbegin \DIFdel{where }\DIFdelend \DIFaddbegin \DIFadd{Here, }\DIFaddend $\psi(\mathbf{r},\mathbf{R})$ is the electronic \DIFdelbegin \DIFdel{wavefunction}\DIFdelend \DIFaddbegin \DIFadd{wave-function}\DIFaddend , and $\chi_{I}(\mathbf{R})$ \DIFdelbegin \DIFdel{represent the ionic wavefunction}\DIFdelend \DIFaddbegin \DIFadd{represents the ionic wave-function}\DIFaddend . Using this \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend and after certain approximations we arrive at,
 \be\label{SE_e}
 \left[ T_E + V_{EE} + V_{IE}\right]\psi(\mathbf{r},\mathbf{R}) = E(\mathbf{R}) \psi(\mathbf{r},\mathbf{R})~.
 \ee
 %
Here, $E(\mathbf{R})$ is the energy of the electrons, considering the ions to be frozen at the location $\mathbf{R}$. Similar equation can be obtained for the ionic \DIFdelbegin \DIFdel{wavefunctions}\DIFdelend \DIFaddbegin \DIFadd{wave-functions}\DIFaddend . However, here we only focus on the electronic part. In Eq.~\ref{SE_e}, although the electronic and ionic \DIFdelbegin \DIFdel{wavefunctios }\DIFdelend \DIFaddbegin \DIFadd{wave-functions }\DIFaddend are decoupled, it is still extremely difficult to solve. Next approximation comes through the Hartree approximation, which assumes an independent electron picture.~\cite{hartree1928} Therefore, within this approximation, the many-body electronic \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend is written as a product of individual single particle \DIFdelbegin \DIFdel{wavefunctions }\DIFdelend \DIFaddbegin \DIFadd{wave-functions }\DIFaddend ($\psi_i$), $i.e.$
\be
\psi_H=\psi_1({\bf r_1},\bm{\sigma_1})\psi_2({\bf r_2},\bm{\sigma_2})....\psi_N({\bf r_N},\bm{\sigma_N})\DIFaddbegin \DIFadd{~,
}\DIFaddend \ee
where $\bm{\sigma}$ denotes the spin of the electrons. This \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend within a variational approach leads to the Hartree equation given by,
\be
\DIFdelbegin %DIFDELCMD < [%%%
\DIFdelend \DIFaddbegin \left[\DIFaddend -\frac{\hbar^2}{2m}\nabla^2+V_{IE}({\bf r})+V_H({\bf r})\DIFdelbegin %DIFDELCMD < ]%%%
\DIFdelend \DIFaddbegin \right]\DIFaddend \psi_i({\bm r})=E_i\psi_i({\bm r})\DIFaddbegin \DIFadd{~,
}\DIFaddend \ee
\DIFdelbegin \DIFdel{where }\DIFdelend \DIFaddbegin \DIFadd{with }\DIFaddend the Hartree potential \DIFdelbegin \DIFdel{$V_H$ is given by:
}\DIFdelend \DIFaddbegin \DIFadd{being, 
}\DIFaddend \be
V_H(\bm{r})=e^2\int \frac{d^3\bm{r'}}{|\bm{r}-\bm{r'}|}\sum_{j\neq i}|\psi_j(\bm{r'})|^2\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{Note that, the }\DIFdelend \DIFaddbegin \DIFadd{The }\DIFaddend Hartree potential is the average electrostatic potential at the location of the $i^{th}$ electron due to all the other electrons in the system. Interestingly, the Hartree potential is directly dependent on the final \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend of the system, and therefore, the equation must be solved \DIFdelbegin \DIFdel{self- consistently}\DIFdelend \DIFaddbegin \DIFadd{self-consistently}\DIFaddend . 

In the case of Hartree equation, the electrons are considered as distinguishable particles. However, in reality, electrons are Fermions, and therefore, the electronic \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend must satisfy antisymmetric property with respect to the exchange of positions and spins. Therefore, the total \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend has to be written as the Slater determinant of the individual \DIFdelbegin \DIFdel{wavefunctions}\DIFdelend \DIFaddbegin \DIFadd{wave-functions}\DIFaddend . This leads to the Hartree-Fock equation, which contains one additional term called the exchange energy term~\cite{fock1930}. This term solely arises due to the indistinguishability of electrons. Note that, both Hartree and Hartree-Fock methods neglect the correlation effects. These methods are usually suitable for small atoms or molecules, and become computationally expensive for large systems. One solution to deal with large systems is the use of density functional theory.

\section{Density functional theory}\label{DFT}
The many-body \DIFdelbegin \DIFdel{wavefunction of an N-electron }\DIFdelend \DIFaddbegin \DIFadd{wave-function of an $N$-electron }\DIFaddend system is a function of \DIFdelbegin \DIFdel{3N }\DIFdelend \DIFaddbegin \DIFadd{$3N$ }\DIFaddend variables. Clearly, dealing with such a large number of variables in the real system is extremely difficult. The idea of DFT is to use the electron density as a fundamental quantity as it only involves three variables (for example, $x,y,z$ coordinates). This idea was formulated in a proper framework by Hohenberg and Kohn in 1964 in terms of two theorems \DIFdelbegin \DIFdel{~}\DIFdelend \cite{hohenberg1964},

\begin{itemize}
\item The external potential, $V_{ext}(\mathbf{r})$, of an interacting many-electron system can be expressed as a unique functional of the ground state density, $n(\mathbf{r})$. Therefore, the ground state energy of this system 
is also a unique functional of $n(\mathbf{r})$, i.e. $E=E[n]$.

\item The total energy functional, $E[n]$, has a minimum equal to ground state energy corresponding to the ground state density, $n(\mathbf{r})$. 
\end{itemize}

\subsection{Kohn-Sham equation}

This problem can be further simplified by mapping the problem of the interacting electrons to an auxiliary non-interacting system which has the same density profile. In this non-interacting system, one can define single-particle orbitals known as the Kohn-Sham orbitals $(\psi^{KS}_i(\bm{r}))$ which reproduces the density of the actual system, 
\be
n(\bm{r})=\sum_{i=1}^N |\psi^{KS}_i(\bm{r})|^2\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{where }\DIFdelend \DIFaddbegin \DIFadd{Here, }\DIFaddend the $\psi^{KS}_i(\bm{r})$ follow the Kohn-Sham equation,
\be
\label{KS}
\DIFdelbegin %DIFDELCMD < \big [%%%
\DIFdelend \DIFaddbegin \left[\DIFaddend -\frac{\hbar^2}{2m}\nabla^2+V^{[n]}_{eff}(\bm{r})\DIFdelbegin %DIFDELCMD < \big ]%%%
\DIFdelend \DIFaddbegin \right]\DIFaddend \psi^{KS}_i(\bm{r})=E_i\psi^{KS}_i(\bm{r}) 
\ee
where, \DIFdelbegin \DIFdel{E$_i$ }\DIFdelend \DIFaddbegin \DIFadd{$E_i$ }\DIFaddend are the Kohn-Sham eigenvalues\DIFdelbegin \DIFdel{, and $\psi^{KS}_i$'s are the Kohn-Sham orbitals}\DIFdelend ~\cite{kohn1965}. Here, the superscript \DIFdelbegin %DIFDELCMD < [%%%
\DIFdel{n}%DIFDELCMD < ] %%%
\DIFdelend \DIFaddbegin \DIFadd{$[n]$ }\DIFaddend denotes that $V_{eff}^{[n]}(\bm{r})$ is a functional of the electron density. Note that, $V_{eff}^{[n]}(\bm{r})$ consists of three terms\DIFdelbegin \DIFdel{,
}\DIFdelend \DIFaddbegin \DIFadd{:
}\DIFaddend \be
V^{[n]}_{eff}(\bm{r})=V_{ext}(\bm{r})+V^{[n]}_H(\bm{r})+V^{[n]}_{XC}(\bm{r})\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{where, the }\DIFdelend \DIFaddbegin \DIFadd{The }\DIFaddend Hartree potential $V^{[n]}_H(\bm{r})$ is given by,
\be
V^{[n]}_H(\bm r)=e^2 \int d^3r' \frac{n(\bf r')}{|\bf r - r'|}\DIFaddbegin \DIFadd{~,
}\DIFaddend \ee
and the exchange-correlation potential, $V_{XC}^{[n]}(\bm{r})$, \DIFaddbegin \DIFadd{is 
}\DIFaddend \be
V_{XC}^{[n]}(\bm{r})=\frac{\delta E_{XC}^{[n]}}{\delta n(\bm{r})}\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{here}\DIFdelend \DIFaddbegin \DIFadd{Here}\DIFaddend , $E^{[n]}_{XC}$  is the exchange-correlation part of the total energy. It's exact form is unknown, and it plays a central role in DFT. Note that, Eqn.~\ref{KS} needs to be solved self-consistently \DIFaddbegin \DIFadd{as $V_{eff}^{[n]}(\bm{r})$ is a functional of the electron density}\DIFaddend . 

Kohn-Sham equation is exact if all the terms in $V^{[n]}_{eff}$ are exactly known. Various approximations of DFT come through the approximations related in calculating the exchange-correlation part of the potential. Two of the most popular approximations in calculating the $V_{XC}$ are the local density approximation (LDA) and generalized gradient approximation (GGA), as discussed in the next section.

\subsection{LDA and GGA}

The simplest approximation, known as LDA, \DIFdelbegin \DIFdel{in calculating the E$_{XC}$ is }\DIFdelend \DIFaddbegin \DIFadd{for calculating the $E_{XC}$ was }\DIFaddend proposed by Kohn and Sham in 1965~\cite{kohn1965}. In this case, it is assumed that the whole electron gas has a slowly varying density profile, n(r). Therefore, the exchange-correlation energy at a small elemental volume $d^3r$ should remain locally uniform. Therefore, within LDA, the $E_{XC}$ for the whole system is given by,
\be
E_{XC}[n]=\int n(\bm{r}) \epsilon\DIFdelbegin \DIFdel{_{XC}(n(}%DIFDELCMD < \bm{r}%%%
\DIFdel{)) }\DIFdelend \DIFaddbegin \DIFadd{_{XC}[n(\bm{r})] }\DIFaddend d^3\bm{r}
\ee
where, \DIFdelbegin \DIFdel{$\epsilon_{XC}(n(\bm{r}))$ }\DIFdelend \DIFaddbegin \DIFadd{$\epsilon_{XC}[n(\bm{r})]$ }\DIFaddend is the exchange-correlation energy per particle for an uniform electron gas of local density $n(\bm{r})$. The form of \DIFdelbegin \DIFdel{$\epsilon_{XC}(n(\bm{r}))$ }\DIFdelend \DIFaddbegin \DIFadd{$\epsilon_{XC}[n(\bm{r})]$ }\DIFaddend is obtained from high-level many-body calculations for a uniform electron gas. For example, the forms developed by Gunnarsson and Lundqvist or Ceperly and Adler are used in many of the current implementations of LDA ~\cite{PhysRevB.13.4274,PhysRevLett.45.566}. LDA generally works well for systems with uniform electron density and therefore yields good results for metals. However, in the case of semiconductors, it underestimates the band gap \DIFdelbegin \DIFdel{$\sim$ }\DIFdelend \DIFaddbegin \DIFadd{upto }\DIFaddend 50\%. 

The next \DIFdelbegin \DIFdel{order }\DIFdelend approximation in computing $E_{XC}$ is called the generalized gradient approximations (GGA) \cite{gga,PW,PBE_sol}. Unlike LDA, GGA includes the first gradient correction of the density. Therefore it also includes the effect \DIFaddbegin \DIFadd{of }\DIFaddend local inhomogeneity of the electron density. Within GGA, the total exchange-correlation energy can be expressed as: 
\be
E_{XC}[n(\mathbf{r})] = \int  n(\mathbf{r})\epsilon_{XC}(n(\mathbf{r}), \mathbf{\nabla}n(\mathbf{r})) d^3\bm{r}~.
\ee
There are several implementations of the GGA, out of which the most famous is the one developed by Perdew, Burke, and Ernzerhof (PBE)\cite{gga}. The other implementations are by Perdew and Wang (PW 91) \cite{PW} and various optimized version of PBE for solids (PBE-sol)\cite{PBE_sol} etc. In certain systems, GGA works better than the LDA scheme. However, both LDA and GGA severely underestimate the bandgap of an insulator~\cite{prasad2013}.

Apart from  LDA and GGA, there are various other methods to calculate the electronic structure of materials, for example, LDA+U, GGA+U scheme, various hybrid functionals like HSE, many-body techniques like GW, etc~\cite{LDA_plus_u,hse_03,Aryasetiawan_1998}. However, in most of the works related to this thesis, we have used the GGA method developed by Perdew, Burke, and Ernzerhof (PBE)\cite{gga}.

There are various approaches to solve the Kohn-Sham equation. In the next section, we describe one of the most popular methods to solve the Kohn-Sham equation with the pseudopotentials using a plane-wave basis set.

\subsection{Plane wave basis set}\label{PWB}
In a crystalline material, the periodic boundary conditions allow the Bloch wave function $(\psi_{nk}(\mathbf{r}))$ to be expanded in a plane wave basis set as,
 %
 \be
 \label{PWB_eqn}
\psi_{ik}(\mathbf{r}) = \sum_{\mathbf{G}} C_{i,\mathbf{k}}^{\mathbf{G}}~ e^{i(\mathbf{k}+\mathbf{G}) \cdot \mathbf{r}}~. 
 \ee
 %
\DIFdelbegin \DIFdel{where}\DIFdelend \DIFaddbegin \DIFadd{Here}\DIFaddend , $\mathbf{G}$ is the reciprocal lattice vector, and $C_{i,\mathbf{k}}^{\mathbf{G}}$ is the expansion coefficient. Ideally, this sum contains an infinte number of plane waves. However, for computational \DIFdelbegin \DIFdel{efficency }\DIFdelend \DIFaddbegin \DIFadd{efficiency }\DIFaddend it  must be restricted to an optimal number of plane waves. In practice, one needs to consider a sphere of radius $|\bf G_{max}|$ in the reciprocal space, keeping the origin at the center, and consider all the ${\bf G}$ vectors which are inside this sphere~\cite{martin2004,prasad2013}. The $|\bf{G_{max}}|$ is obtained from the kinetic energy cutoff ($E_{cut}$) using the following equation,
 \be
 E_{cut} = \frac{\hbar |\bf{k+G_{max}|^2}}{2m}.
 \ee 


%Calculation of many quantities are generally associated with a BZ integration. This is done by replacing the integration with a discrete summation. In this regard, the tetrahedron method is very useful. In practice, a BZ is divided into smaller symmetry-related parts, and the final sum is performed only within a smaller region of the BZ called the irreducible BZ for computational efficiency.

 \subsection{Pseudopotential}\label{Pseudo_pot}
The \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend of the valence electrons must satisfy the orthogonality condition with the core electron \DIFdelbegin \DIFdel{wavefunctions}\DIFdelend \DIFaddbegin \DIFadd{wave-functions}\DIFaddend . This results in a rapidly oscillating valance electron \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend in the core region. Therefore, a large number of plane waves are needed in Eqn.~\ref{PWB_eqn} to properly describe the valence electron \DIFdelbegin \DIFdel{wavefunction}\DIFdelend \DIFaddbegin \DIFadd{wave-function}\DIFaddend . Since the computational cost increases with the number of plane waves, an efficient approach to solve the problem is the use of pseudopotentials~\cite{martin2004,prasad2013}.

Let us consider that the actual \DIFdelbegin \DIFdel{wavefunction }\DIFdelend \DIFaddbegin \DIFadd{wave-function }\DIFaddend of the system satisfies the Kohn-Sham equation:
\be\label{KS_eq}
\left[-\frac{\hbar}{2m}\nabla^2 + \DIFdelbegin \DIFdel{v}\DIFdelend \DIFaddbegin \DIFadd{V}\DIFaddend _{eff}(\mathbf{r})\right]\psi_i({\mathbf{r}})=E_i \psi_i({\mathbf{r}})~,
\ee
One can construct the pseudo \DIFdelbegin \DIFdel{wavefunction}\DIFdelend \DIFaddbegin \DIFadd{wave-function}\DIFaddend , $\phi_i$, such that,
\be
\psi_i({\bf r})=(1-P)\phi_i({\bf r})
\ee
where the projection operator P is given by,
\be
P=\sum_j |\bm{k_j} \rangle \langle\bm{k_j}|
\ee
Note that, P projects any function to the core states $(|\bm{k_j} \rangle)$.
It can be shown that $\phi_i({\bf r)}$ satisfies a similar equation as $\psi_i({\bf r})$:
\be\label{KS_psudo}
\left[-\frac{\hbar}{2m}\nabla^2 + W(\mathbf{r})\right]\phi_i({\mathbf{r}})=E_i \phi_i({\mathbf{r}})~,
\ee
where $W(\bm{r})$ is the pseudo potential and it can be expressed as:
\be
W=V_{eff}({\bf r})-[-\frac{1}{2}\nabla^2+V_{eff}({\bf r})]P+E_iP
\ee
Note that, Eqn.~\ref{KS_psudo} yields the same eigenvalues as the actual equation. However, since the core states are already projected out of $\phi_i$, it is generally a smooth function and can be reproduced using a smaller set of plane waves. The pseudo wavefunction generally mimics the true wavefunction beyond a cutoff radius.

There are two widely used methods to calculate pseudopotentials; one is the norm-conserving approach developed by Kleinman and Bylander \cite{kleinman1982}, and the other is the ultrasoft method developed by Vanderbilt \cite{vanderbilt1990}. In the case of norm-conserving pseudopotential, the norm of the actual wavefunction must reproduce the norm of the pseudo wavefunction within the cutoff radius. However, in the case of ultrasoft pseudopotential, this restriction is not maintained. An ultrasoft pseudo wavefunction generally requires a lower kinetic energy cutoff i.e., it can be constructed using a smaller number of plane waves. These type of pseudopotentials are used in codes like Quantum ESPRESSO.~\cite{Giannozzi_2009}

Apart from the pseudopotential method, there is projector augmented wave (PAW) method, which lies in between the all-electron potential and the pseudopotential ~\cite{paw}. In this method, the wavefunction is divided into two parts, a partial-wave expansion within an atom centered sphere, and a pseudo wavefunction outside the augmented region. Therefore, PAW methods are better because they consider both the core electrons and, at the same time, uses the pseudopotential method to deal with the valance electrons. PAW potential is generally used in codes like VASP, GPAW.~\cite{vasp,PhysRevB.71.035109}


\section{Wannier function based modeling}\label{wann}
In a tight-binding model, the Bloch wavefunction is generally expressed as a linear combination of localized orbitals~\cite{ashcroft1976solid,vanderbilt2018berry}. This yields an accurate description of the electronic structure with much higher computational efficiency. In recent times, the Wannier function based tight-binding method has \DIFdelbegin \DIFdel{been }\DIFdelend proven to be \DIFdelbegin \DIFdel{one of the most powerful ways }\DIFdelend \DIFaddbegin \DIFadd{a  powerful way }\DIFaddend to explore topological materials~\cite{wannier,Bansil16}. This method is not restricted to the nearest neighbor or next nearest neighbor hoppings, rather many smaller hoppings are also taken into account to describe the electronic structure with great accuracy. As discussed earlier, DFT based techniques have been extremely successful in recent times in dealing with properties that require a coarse-grained sampling of the BZ. However, in the case of topological materials, it often becomes essential to sample the Brillouin zone in a much denser \DIFdelbegin \DIFdel{k-grid}\DIFdelend \DIFaddbegin \DIFadd{$k$-grid}\DIFaddend . For example, if one intends to find the Weyl points, which can be located anywhere in the BZ, it is necessary to sample the BZ in a very dense \DIFdelbegin \DIFdel{k-grid}\DIFdelend \DIFaddbegin \DIFadd{$k$-grid}\DIFaddend . Similarly, for the calculation of the Berry phase/curvature, it becomes essential to sample the BZ in a dense \DIFdelbegin \DIFdel{k-grid}\DIFdelend \DIFaddbegin \DIFadd{$k$-grid}\DIFaddend . Wannier function based tight-binding modeling is one solution to this problem. The idea of a Wannier function based tight-binding method is to extract the real space hopping parameters only for a limited number of relevant bands around the Fermi energy~\cite{wannier}. Using these real space hopping parameters, one can construct the \DIFdelbegin \DIFdel{k-space }\DIFdelend \DIFaddbegin \DIFadd{$k$-space }\DIFaddend Hamiltonian, which has a much smaller size (typically $\sim 100\times 100$ matrix at each k-points). In the following section, we discuss various properties of the Wannier functions.

Wannier functions can be considered as the Fourier transform of the Bloch functions~\cite{PhysRev.52.191,wannier,RevModPhys.84.1419,vanderbilt2018berry}. The Wannier functions associated with the $n^{th}$ Bloch band, $\psi_{nk}$, can be constructed as 
\be
W_{n{\bf R}} = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} e^{-i\bf{k.R}} \psi_{n{\bf k}}  d^3k\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee 
\DIFdelbegin \DIFdel{where}\DIFdelend \DIFaddbegin \DIFadd{Here}\DIFaddend , ${\bf R}$ is the unit cell index, and $V_{cell}$ is the unit cell volume. Note that, since $\psi_{nk}(\bm{r})$ has a gauge freedom\DIFdelbegin \DIFdel{and }\DIFdelend \DIFaddbegin \DIFadd{, }\DIFaddend it can be made smooth over the Brillouin zone by choosing a suitable gauge. This fact ensures that $W_{n{\bf R}}$ decays rapidly with $|{\bf r-R}|$. Therefore, Wannier functions are generally well localized in real space. Moreover, Wannier functions are orthogonal to each other in the real space, i.e.
\be
\langle W_{m\bf R}|W_{n\bf R'} \rangle =\delta_{mn}\delta_{\bf RR'}\DIFaddbegin \DIFadd{~,
}\DIFaddend \ee
and they span the same Hilbert space as the Bloch functions. The matrix elements for the Hamiltonian in the Wannier basis can be written as 
\be
H_{mn}({\bf R})=\langle W_{m\bf R} |H|W_{n\bf R}\rangle\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
Once these real space hopping elements are obtained, one can find the $k$-space Hamiltonian as:
\be
H_{mn}({\bf k})=\sum_{\bf R} e^{i\bf k.R} H_{mn}({\bf R}) 
\ee
or 
\be
H_{mn}({\bf k})=\sum_{\bf R} e^{i\bm{ \bm {k.(R+\tau_m-\tau_n)}}} H_{mn}({\bf R}) 
\ee
where $\bm{\tau_n}$ represents the location of the $n^{th}$ Wannier orbital in the home unit cell. The eigenvalues of both these constructions are the same, but their eigenvectors are different. The first one correspond to the Bloch \DIFdelbegin \DIFdel{wavefunctions }\DIFdelend \DIFaddbegin \DIFadd{wave-functions }\DIFaddend , $\psi_{nk}$, while the second convention yields the periodic part of the Bloch wave function, $u_{n{\bf k}}(r)=\psi_{n{\bf k}}(r)e^{-ik.r}$.~\cite{vanderbilt2018berry} The second formalism is generally more suitable in the context of topological materials because it is directly related to the Berry phase and Berry curvature. 

Wannier functions can be used to calculate various properties. For example, the Berry phase of a system can be calculated using the matrix element of the position operator in the following way:

\be
\overline{\mathbf{r}}_n = \la w_{n0}| \mathbf{r} | w_{n0}\ra = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} \la u_{n\mathbf{k}} | i \nabla_{\mathbf{k}} u_{n\mathbf{k}}\ra d^3\bm{k}\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{or, in }\DIFdelend \DIFaddbegin \DIFadd{In }\DIFaddend one dimension, \DIFaddbegin \DIFadd{we have 
}\DIFaddend \be
\overline{x}_n = (a/2\pi) \int_0^{2\pi} \la u_{nk} | i \partial_{k} u_{nk}\DIFaddbegin \DIFadd{~
}\DIFaddend \ra dk\DIFaddbegin \DIFadd{~,
}\DIFaddend \ee
or,
\be
\overline{x}_n = a \frac{\phi_n}{2\pi}\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
\DIFdelbegin \DIFdel{where}\DIFdelend \DIFaddbegin \DIFadd{Here}\DIFaddend , $\phi_n$ represents the Berry phase and $a$ is the cell \DIFdelbegin \DIFdel{parameters }\DIFdelend \DIFaddbegin \DIFadd{parameter }\DIFaddend of the one-dimensional lattice. Therefore, the information about the Berry phase can be easily obtained by tracking the Wannier charge centers \cite{vanderbilt2018berry}. Another important use of the Wannier function based Hamiltonian is the calculation of the surface states as discussed in the next section.

\subsection{Surface states using the Wannier Hamiltonian}
A topological system generally hosts protected surface states due to the bulk boundary \DIFdelbegin \DIFdel{correspondance}\DIFdelend \DIFaddbegin \DIFadd{correspondence}\DIFaddend . There are two popular ways to study the surface states within the Wannier function based formalism. They are, (i) surface state in a finite-sized slab geometry and (ii) surface state in a semi-infinite geometry~\cite{Wu2017}. In both the cases, there are two periodic directions which are parallel to the surface. The third direction which is perpendicular to the surface breaks the translation symmetry and the momentum is not a good quantum number along this direction. A slab Hamiltonian can be constructed systematically by considering layers stacked 
along the perpendicular direction. The slab Hamiltonian for $n_{slab}$ layers along the 2D momentum $\bf{k}_{\|}$ can be written as,
\be\label{Slab_Ham}
H^{slab}_{mn}(\bf{k}_{\|}) = \left(\begin{matrix}
H_{mn, 11} (\bf{k}_{\|}) & H_{mn, 12} (\bf{k}_{\|}) & \cdots & H_{mn, 1 n_{slab}} (\bf{k}_{\|})  \\
H_{mn, 21} (\bf{k}_{\|}) & H_{mn, 22} (\bf{k}_{\|}) & \cdots & H_{mn, 2 n_{slab}} (\bf{k}_{\|})  \\
\vdots & \vdots & \ddots & \vdots \\
H_{mn, n_s 1} (\bf{k}_{\|}) & H_{mn, n_s 2} (\bf{k}_{\|}) & \cdots & H_{mn, n_{slab} n_{slab}} (\bf{k}_{\|})  \\
\end{matrix}
\right).
\ee
Here, the elements in Eq.~\ref{Slab_Ham} are be obtained as,
\be
H_{mn, ij} ({\bf k}_{\|}) = \sum_{{\bf R} = \{\mathbf{R}_{\parallel}, (1-\delta_{ij}) \mathbf{R}_\perp \}}  e^{i \mathbf{k_{\|}} \cdot \mathbf{R}} H_{mn}(\mathbf{R}) .
\ee 
By diagonalizing the Hamiltonian in Eq.~\ref{Slab_Ham}\DIFaddbegin \DIFadd{, }\DIFaddend one can obtain the energy bands for the slab system. In order to obtain the density of states one can use the Green's function method:
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdelend %DIF > 
\be
G^{slab}({\omega,\bf k})=\frac{1}{(\omega+i\eta)\mathbb{1}-H_{slab}}\DIFaddbegin \DIFadd{~.
}\DIFaddend \ee
Here, $\mathbb{1}$ is the identity matrix of dimension equal to the dimension of the slab Hamiltonian, $H_{slab}$. The surface spectral function can be obtained as,
\be
A(\mathbf{k}_{\|},\omega) = - \frac{1}{\pi} \lim_{\eta \to 0^+} \mathrm{Im~Tr} [G^{slab}_{11}(\mathbf{k}_{\|}, \omega+i \eta )]. 
\ee
Here, $G^{slab}_{11}$ corresponds to the block that belongs to the surface layer.

The second method is to calculate the surface states for a semi-infinite system using the method of iterative surface Green's function. In this method one defines a principle layer which are stacked along the vertical \DIFdelbegin \DIFdel{direcion}\DIFdelend \DIFaddbegin \DIFadd{direction}\DIFaddend . The principle layers are chosen such that only the interaction between two adjacent principle layer is non-zero, while the next nearest neighbour interaction terms vanish. If $H_{00}(\mathbf{k}_{\|})$ represents the intralayer $k-$space Hamiltonian and $H_{01}(\mathbf{k}_{\|})$ denotes the inter principle layer coupling, the surface Green's function can be obtained using the Sanchos algorithm~\cite{sancho1985highly} by iteratively solving the following equations:

\bearr \nn \label{SGF-cond}
\alpha_i &=& \alpha_{i-1} (\omega - \epsilon_{i-1})^{-1} \alpha_{i-1}\\ \nn
\beta_i &=& \beta_{i-1} (\omega - \epsilon_{i-1})^{-1} \beta_{i-1}\\ 
\epsilon_{i} &=& \epsilon_{i-1} + \alpha_{i-1} (\omega - \epsilon_{i-1})^{-1} \beta_{i-1} + \beta_{i-1} (\omega - \epsilon_{i-1})^{-1} \alpha_{i-1}\\ \nn
\epsilon_{i}^s &=&  \epsilon^s_{i-1} + \alpha_{i-1} (\omega - \epsilon_{i-1})^{-1} \beta_{i-1}\\ \nn
\tilde{\epsilon}_{i}^s &=&  \tilde{\epsilon}^s_{i-1} + \beta_{i-1} (\omega - \epsilon_{i-1})^{-1} \alpha_{i-1}~. \nn
\eearr 
The iterations start with the initial values,
\bearr  \label{SG}
\epsilon_0 &=& \tilde{\epsilon}_0 = \tilde{\epsilon}^s_0 = H_{00}(\mathbf{k}_{\|})\\ \nn
\alpha_0 &=& H_{01}(\mathbf{k}_{\|})\\ \nn
\beta_0 &=& H^{\dagger}_{01}(\mathbf{k}_{\|})\DIFaddbegin \DIFadd{~.
}\DIFaddend \eearr 
The convergence in Eq.~\ref{SGF-cond} is obtained after $n^{th}$ iteration when $\epsilon_n=\epsilon_{n-1}$ or $\tilde{\epsilon}_n = \tilde{\epsilon}_{n-1}$, within the numerical accuracy. This method is highly convergent, and for a typical system it converges within  $\sim 20$ steps.
The projected bulk Green's functions and final surface Green's function in  two dual surfaces are obtained as,
\bearr \
G_s(\mathbf{k}_{\|},\omega) &=& (\omega - \epsilon^{s}_n)^{-1}\\ \nn
\tilde{G}_s(\mathbf{k}_{\|}, \omega ) &=& (\omega - \tilde{\epsilon}^{s}_n)^{-1}\\ \nn
G_{\rm bulk}(\mathbf{k}_{\|},\omega) &=& (\omega - \epsilon_n)^{-1} ~.\\ \nn
\eearr
The surface spectral function can be obtained as,
\be
A(\mathbf{k}_{\|},\omega) = - \frac{1}{\pi} \lim_{\eta \to 0^+} \mathrm{Im~Tr} [G_s(\mathbf{k}_{\|}, \omega+i \eta )]. 
\ee
The spin texture of the surface states can be calculate using the following equation\DIFdelbegin \DIFdel{:
}\DIFdelend \DIFaddbegin \DIFadd{, 
}\DIFaddend \be
\bm{S} (\mathbf{k}_{\|},\omega) = - \frac{1}{\pi} \lim_{\eta \to 0^+} \mathrm{Im~Tr} [{\bm \sigma}G_s(\mathbf{k}_{\|}, \omega+i \eta )]/A(\mathbf{k}_{\|},\omega). 
\ee
\DIFdelbegin %DIFDELCMD < 

%DIFDELCMD < %%%
\DIFdel{where }\DIFdelend \DIFaddbegin \DIFadd{Here, }\DIFaddend $\bm{\sigma}$ is the Pauli spin matrix. A detailed description about the Wannier functions can be found in Ref.~\cite{RevModPhys.84.1419}. In most of the work related to this thesis, the real space Wannier Hamiltonians are obtained using the Wannier90 code \cite{wannier90}. We use various inhouse codes along with the WannierTools package for exploring various topological properties~\cite{Wu2017}.

To summarize, in this chapter, we have provided a brief overview of the methods that we use to explore topological materials. Various parameters used for DFT and Wannier models (for example, kinetic energy cutoff, $k-$grid information, specific projections used to build a Wannier model, etc.) will be presented in the respective chapters.

==> synopsis.tex <==
% !TEX root = thesis_revised.tex

\thispagestyle{fancy}
\makeatletter%
\long\def\@makefnmark{%
	\hbox {{\normalfont \@thefnmark }}}%
\makeatother


\makeatletter%
\long\def\@makefntext#1{%
	\parindent 1.5em\noindent \hb@xt@ 1.5em{\hss [\@makefnmark] }#1}%
\makeatother

\centerline{\Huge\bf Synopsis}
\vskip 1.0cm 
\begin{quote}
	\begin{tabular}[]{p{5.5cm}cp{9.0cm}}
		Name				&:	&{\bf Pushpendra Kumar Yadav}\\[0.5em]
		Roll No.			&:	&{\bf 18209268 }\\[0.5em]
		Degree for which submitted	&:	&{\bf Doctor of Philosophy}\\[0.5em]
		Department			&:	&{\bf Physics}\\[0.5em]
		Title of the Thesis 		&:	&{\bf Exciton dynamics in equilibrium}\\
		& &{\bf and nonequilibrium regimes}\\
		
		\\
		
		Thesis Supervisor		&:	&{\bf Prof. Amit Agarwal} \\ 
		\\[0.5em]
		
		%		\\
		Month and year \\ of submission	&:	&{\bf February, 2024}\\[0.0em]
	\end{tabular}
\end{quote}
\hrule
%\hrulefill
\vskip 1.0 cm

Interaction among the photo-excited electrons and holes in an insulating solid leads to the formation of a bound state of an electron-hole pair called exciton~[\footnote{{L. J. Sham and T. M. Rice}, {\em Phys. Rev.}, {\bf 144}, 708~(1966)}, \footnote{{G. Strinati}, {\em Phys. Rev. B}, {\bf 29}, 5718~(1984)}]. The excitons govern most of the optical responses and explain several fundamental phenomena in condensed matter. By incorporating the electron-hole correlations at absolute zero temperature and low electron-hole pair density in the excited state, \textit{ab-initio} based theoretical study of optical excitations predict reasonably accurate optical absorption and emission [\footnote{{M. S. Hybertsen and S. G. Louie}, {\em Phys. Rev. Lett.}, {\bf 55}, 1418~(1985)}]. However, some recent experiments have probed the impact of exciton-exciton interactions by increasing the pump fluence or photo-excited carrier density, bringing the electron-hole system into a nonequilibrium regime [\footnote{{Sie, E. J. {\em et. al.}}, {\em Nano Lett.}, {\bf 17}, 7, 4210–4216~(2017)}]. At finite temperatures, within the nonequilibrium regime, the electron-hole system has been reported to exhibit electron-hole plasma and electron-hole liquid phase in the density-temperature parameter space~[\footnote{{Arp T. B., {\em et. al.}}, {\em Nat. Photon.}, {\bf 13}, 245~(2019)}]. However, the theoretical understanding of these exciting experiments in the nonequilibrium regime is yet to be explored.

In this thesis, we demonstrate the presence of bound excitons in atomically thin two-dimensional materials from first-principle based approach. We estimate the single-particle energies using the GW (where $G$ stands for the single-particle Green's function and $W$ represents the screened Coulomb potential) approximation (GWA) and incorporate the electron-hole correlations via the Bethe-Salpeter equation (BSE). The fundamentals of excitons have been studied in the low excitation density, i.e., in the equilibrium limit. With increasing photo-excited carrier density, we show that the lowest energy exciton in monolayer MoSi$_2$Z$_4$ (Z = N, P, As) follows the redshift-blueshift crossover due to the renormalized exciton binding energies in the nonequilibrium regime. Further, we study temperature-dependent optical absorption and photoluminescence (PL) phenomenon in monolayer aluminum nitride (AlN) in the equilibrium regime. We find that electron-phonon interactions significantly modify the electronic energy, excitonic absorption, emission spectrum, and exciton lifetime. At low temperatures, the PL emission signals exhibit full excitonic thermalization with phonon replica below the indirect exciton energy. Finally, we combined the impact of temperature and electron-hole density and investigated a photo-excited electron-hole system in the nonequilibrium regime. We show that photo-excited electrons and holes in insulators above a critical density and below a critical temperature can condense to form an electron–hole liquid (EHL) phase. However, observing the EHL phase at room temperature is extremely challenging. Here, we propose the monolayer MoSi$_2$Z$_4$ (Z = N, As, P) series of compounds as promising platforms for observing the EHL phase at room temperature. Stronger effective Coulomb interactions in two dimensions help these monolayers stabilize the EHL phase with increased EHL binding energy, transition temperature, and strongly bound excitons. 
%Our findings motivate further exploration of two-dimensional semiconductors for realizing the EHL phase at high temperatures and harness collective phenomena for optoelectronic applications.

In Chapter \ref{chap1}, we introduce the fundamentals of the exciton quasiparticles generated upon optical excitation in insulating materials and their impact on different physical observables in condensed matter. A brief discussion about the types of excitons, the effect of dimensionality, and screening on exciton binding energies follows this. Next, we classify excitons based on optical selection rules as bright and dark excitons and based on their interaction with other charged particles or excitons, such as trion and biexciton complexes and electron-hole droplets. In the latter part of the chapter, we discuss the importance of exciton physics in two-dimensional materials and their usefulness in next generation optoelectronic devices. Briefly, we also discuss the theoretical methods adopted for studying optical excitations in this thesis.

In Chapter \ref{chap2}, we discuss the different formalisms used to explore the electronic structures and optical excitations using first-principles methods. We review the many-body Hamiltonian and its solution within the density functional theory (DFT). Further, to incorporate the electron-self energy, we have adopted the GWA to estimate the quasiparticle energies of photo-excited electrons and holes. This is followed by a discussion on the interaction between optically excited electrons and holes leading to the exciton formation and a calculation of the exciton energies and coupled electron-hole wavefunction utilizing the BSE. Furthermore, to understand the effect of lattice vibrations on optical excitations, we follow the electron-phonon interaction calculation within the density functional perturbation theory and obtain electron-phonon matrix elements. The electron-phonon interaction effects are finally applied to the quasiparticles (electron, hole, and excitons) energy correction, and the role of phonon momentum is utilized to understand the indirect photon emission in the indirect bandgap materials. 


In Chapter \ref{chap3}, we investigate the exciton quasiparticle generated in synthetic monolayers of MoSi$_2$N$_4$, MoSi$_2$As$_4$, and MoSi$_2$P$_4$, upon optical excitation. Going beyond the equilibrium properties, we study the fluence-dependent optical spectra and the emergence of exciton–exiton interaction in the nonequilibrium regime for MoSi$_2$N$_4$.
We unveil the renormalization of the exciton binding energy (BE) of the $A$ and $B$ exciton peaks with increasing photo-generated carrier density in the MoSi$_2$N$_4$ monolayer. The exciton BE shows a redshift with increasing pump fluence or photo-excited charge carrier density. This decrease in the BE arises from screening the excitonic Coulomb potential by the
photo-excited charge carriers. However, the exciton binding energies show a blueshift crossover on further increase in the pump fluence or exciton density. This establishes that excitons in the MoSi$_2$N$_4$ series display an atom-like attractive and repulsive interaction depending on the inter-exciton separation. Furthermore, for the direct band gap MoSi$_2$As$_4$ and
MoSi$_2$P$_4$ monolayers, we accurately predict the fundamental quasiparticle (QP) and optical band gaps with their detailed excitonic character.

In Chapter \ref{chap4}, we predict the impact of electron-phonon coupling on optical absorption, PL emission, and indirect emission mechanism. We utilize first-principle calculations and calculate temperature-dependent optical properties of a planar AlN monolayer. Our investigation demonstrated the effect of electron-phonon (el-ph) interactions, leading to significant renormalization of quasiparticle energies. Specifically, the calculated optical absorption spectra showcases a redshift and decreased dipole oscillator strengths due to the interplay between electronic and vibrational states. Furthermore, we observe phonon-assisted indirect PL emission within the excitonic framework in the ultraviolet regime. The PL emission sustains at higher temperatures ( $\ge$ 300 K). Furthermore, the highlighted role of exciton-phonon interactions extends beyond AlN, emphasizing their importance in group-III nitrides and other two-dimensional materials. 


In Chapter \ref{chap5}, we establish potential observation of the EHL phase at room temperature within the monolayer {\formulaN} family. Because of the dimensional confinement and reduced dielectric constant, the monolayer {\formulaN} family host strongly bound excitons with exciton binding energy of the order of 1 eV, as discussed in Chapter 3. Since the critical temperature of the EHL phase depends directly on the exciton binding energy ($T_c \sim 0.1E_b$), and therefore {\formulaN} family host EHL phase above a critical exciton density ($n_c$). This prediction marks a significant departure from conventional limitations associated with cryogenic conditions, introducing the observation of the EHL phase in these materials at room temperature. The higher impact of the Coulomb interactions in two dimensions helps these monolayers support the EHL phase with an increased EHL binding energy and transition temperature, along with strongly bound excitons. Our findings motivate further exploration of the {\formula} monolayers for realizing the EHL phase at high temperatures to harness collective
phenomena for optoelectronic applications. %In another experimental collaborative study, we predict the EHL phase in bulk CsPbBrI$_2$ nanocrystals at room temperature. The stability of the EHL phase in the bulk CsPbBrI$_2$ is supported by the strong electron-phonon interaction, leading to strong electron-hole correlation effects. Furthermore, our study will hopefully broaden the understanding of carrier dynamics in ﬂourishing metal-halide perovskite material and {\formula} monolayers, which will help to enhance the light-matter interaction in photovoltaics, optoelectronic devices.


Finally, we summarize the main findings of our work in Chapter \ref{chap6}, followed by a discussion of future prospects.


==> temp.tex <==
Even though DFT offers a reasonably accurate description of the electronic properties, a more simplified approach is often required to obtain physical and chemical understanding of crystalline systems without involving expensive computation. In such cases, the localized-orbital based tight-binding method is extensively adopted. The Wannier functions  \cite{wannier1937} are the Fourier transformed partner to the periodic Bloch functions, and they provide a natural extension to the concept of localized atomic orbital. 
These are exponentially localized functions in the real space and are periodic images of one another. Since they are constructed from the Bloch functions, they span the same subspace of the Hilbert space. However, in contrast to the atomic orbitals, Wannier functions are mutually orthonormal to each other and this turn out to be of great advantage when using second quantization. The detail descriptions of the construction of maximally localized Wannier function (MLWF) based tight binding model can be found in  Refs.~\cite{marzari2012maximally,mostofi2014updated}. In the rest of this section, we discuss some useful properties of  MLWF for isolated bands and construct the Hamiltonian for a slab system starting from the Wannier Hamiltonian. 

If we have an isolated energy band $E_n(\mathbf{k})$, which never crosses other bands in the BZ from above or below, then it can be considered as a smooth and periodic function of $\mathbf{k}$ in 3D reciprocal space. For the Bloch's function $|\psi_{n\mathbf{k}}\ra$ associated with this band, we can define the Fourier transform as, 
%It is then natural to consider its Fourier transform in real space as,
%%
%\be
%E_{n\mathbf{R}} = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} e^{-i\mathbf{k}\cdot \mathbf{R}} E_{n\mathbf{k}} d^3k ~.
%\ee
%%
%The inverse Fourier transform is simply given by, 
% %
%\be
%E_{n\mathbf{k}} = \sum_{\mathbf{R}} e^{i\mathbf{k}\cdot \mathbf{R}} E_{n\mathbf{R}} .
%\ee
%%
%Now suppose we can choose a smooth and periodic gauge for the Bloch's function $|\psi_{n\mathbf{k}}\ra$ associated with this band. We can define the Fourier transform for ,
%
\be \label{Wann_func}
| w\ra_{n\mathbf{R}} = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} e^{-i\mathbf{k}\cdot \mathbf{R}} |\psi \ra_{n\mathbf{k}} d^3k ~.
\ee 
Here, $| w\ra_{n\mathbf{R}}$ is the Fourier transform partner of the Bloch's function and it is known as the \textit{Wannier function} associated with band $n$. The Wannier function $| w\ra_{n\mathbf{R}}$  is centerd near $\mathbf{R}$ and decays rapidly with $|\mathbf{r}-\mathbf{R}|$. 
The inverse Fourier transform is simply given by, 
 %
\be
|\psi \ra_{n\mathbf{k}} = \sum_{\mathbf{R}} e^{i\mathbf{k}\cdot \mathbf{R}} | w\ra_{n\mathbf{R}}  .
\ee
%

\subsection{Properties of Wannier functions}

The Wannier function has the following interesting and useful properties,

\begin{enumerate}
\item Wannier functions are localized in real space, i.e, 
%
\be \nn
| w_{n\mathbf{R}} (\mathbf{r}) | \rightarrow 0 ~~~~\mathrm{as}~~~|\mathbf{r}-\mathbf{R}| ~~\mathrm{becomes~large}~. 
\ee
%
Therefore we can think that Wannier functions are packed in cell $\mathbf{R}$, though their tail can extend to the neighbouring cell.

\item The Wannier functions are translational image of each other. i.e,
%
\be
w_{n\mathbf{R}} (\mathbf{r}) = w_{n\mathbf{R}} (\mathbf{r}-\mathbf{R}).
\ee
%
\item The Wannier functions form an orthonormal set.
%
\be
\la w_{n\mathbf{R}}| w_{n\mathbf{R}^{\prime}}\ra = \delta_{\mathbf{R}\mathbf{R}^{\prime}}
\ee
%
\item The Wannier functions span the same subspace of the Hilbert's space as the Bloch's function from which they are constructed. The projection operator is then defined as,
%
\be
P_n = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} |\psi_{n\mathbf{k}}\ra\la \psi_{n\mathbf{k}} | d^3k = \sum_{\mathbf{R}} |w_{n\mathbf{R}}\ra\la w_{n\mathbf{R}} | .
\ee
%
\item The Hamiltonian matrix elements between the Wannier functions are band diagonal, and these diagonals are none other than the coefficient $E_{n\mathbf{R}}$ (the Fourier transform of the band energies), 
%
\be
\la w_{n0}| H | w_{n\mathbf{R}}\ra = E_{n\mathbf{R}}~.
\ee
%
It implies that the Wannier functions provide an exact tight binding representation of the dispersion $E_{n\mathbf{k}}$ of band $n$. We can construct a tight-binding model consisting of one orbital per cell having an on-site energy $E_{n0}$ and an energy $E_{n\mathbf{R}}$ for hopping to its neighbour located at cell $\mathbf{R}$. This method of reproducing the band structure with high accuracy, using Wannierized tight-binding representation, is known as \textit{Wannier interpolation}.

\item  The matrix element of the position operator between Wannier functions is related to the Berry-phase of the system. 
The position matrix elements between Wannier functions is given by,
%
\be \label{Wann_pos}
\la w_{n0}| \mathbf{r} | w_{n\mathbf{R}}\ra = \mathbf{A}_{n\mathbf{R}}~,
\ee 
%
where $\mathbf{A}_{n\mathbf{R}}$ is the Fourier transform coefficient of the Berry connection $\mathbf{A}_{n}(\mathbf{k})$: 
%
\be \label{Berry_FT}
\mathbf{A}_{n\mathbf{R}} = \frac{V_{cell}}{(2\pi)^3} \int_{BZ} e^{-i\mathbf{k}\cdot \mathbf{R}} \mathbf{A}_{n}(\mathbf{k}) d^3k~.
\ee
%
This allows us to define an important quantity, the Wannier charge center:
% An specially important quantity can be derived from this, which is Wannier charge center and can be written as,
%
\be
\overline{\mathbf{r}}_n = \la w_{n0}| \mathbf{r} | w_{n0}\ra ~.
\ee
% 
From Eq.~\ref{Wann_pos} and Eq.~\ref{Berry_FT} we will get,
%
\bearr \nn
\overline{\mathbf{r}}_n &=& \frac{V_{cell}}{(2\pi)^3} \int_{BZ} \mathbf{A}_{n}(\mathbf{k}) d^3k \\ 
&=& \frac{V_{cell}}{(2\pi)^3} \int_{BZ} \la u_{n\mathbf{k}} | i \nabla_{\mathbf{k}} u_{n\mathbf{k}}\ra d^3k.
\eearr
%
This is nothing but the BZ average of the Berry connection. In one dimension, it  becomes $\overline{x}_n = (a/2\pi) \int_0^{2\pi} \la u_{nk} | i \partial_{k} u_{nk}\ra dk$ or $\overline{x}_n = a \frac{\phi}{2\pi}$. Therefore the Wannier charge center is proportional to the Berry phase $\phi$ by a scale factor $\frac{a}{2\pi}$. This simply means that if the Berry phase evolves from $0$ to $2\pi$, it corresponds to Wannier charge center shift by a lattice constant from $0$ to $a$. This connection between the Berry phase and the Wannier charge center is of immense computational importance for determining the topological phases of matter.
\end{enumerate}


==> tsc.tex <==
Theoretically in an intrinsic topological superconductor with spin-less p+ip type superconducting paring can hold Majorana zero mode in the vortices. 

Nevertheless the reported p-wave superconductor are rare.  (Sr2RuO4, Rev Mod Phys.)

On the other hand the topological superconductivity can arises in an equivalent p+ip superconductor, such as the interface of TI and s-wave conventional superconductor. In this case the proximity effect can induce superconductivity on the spin helical topological surface states.

But to prepare such high quality heterostructure is a huge challenge.

Therefore the alternative approach to realize topological superconductivity is to search equivalent p+ip type superconductivity in a single compound, where the bulk is a s-wave superconductor but host topological surface states that crosses the Fermi energy. 

There are two strategies:
1.  Induce superconductivity in the topological insulator by charge doping such as Cu/Sr/Nb doped Bi2Se3.
2. Search topological properties in existing superconductor. Such as beta-PdBi2, PdTe2, PbTaSe2, Fe(Te0.55Se0.45)

